Binarization as an Attack Surface in Weightless Neural Networks

Weightless Neural Networks (WNNs) are lightweight classifiers that binarize their inputs and learn by storing binary patterns in lookup memories, which makes them attractive for resource-constrained tasks such as intrusion detection. Because a small perturbation that crosses no binarization threshold leaves the binary input unchanged, WNNs may appear naturally robust to adversarial examples; a perturbation that does cross a threshold, however, can still change the prediction. We study this tension in WiSARD, the canonical RAM-based WNN, and in two variants that replace its memories with Bloom filters, Bloom WiSARD and BTHOWeN. A continuous perturbation reaches these classifiers only by crossing an encoding threshold, changing at least one binary tuple, and redirecting a memory query; we formalize this mechanism with a threshold-crossing bound and a response-margin certificate for standard Boolean WiSARD. Controlled MNIST experiments compare linear and data-driven thermometer encodings under model-agnostic sensitivity probes, a score-based Simulated Annealing attack, and surrogate-transfer attacks. Changing only the encoding while keeping each model otherwise fixed shows that encoding granularity can trade a small clean-accuracy loss for a large decrease in attack success. On the Bot-IoT, CICIDS, and UNSW-NB15 intrusion-detection datasets, adversarial perturbations lead WNN detectors to classify many attacks as normal traffic and to raise false alarms, even when their aggregate accuracy remains high.

==> corrected_ids_tables.tex <==
 % Table 6 (linear+Gaussian; FGSM, Random L2, Random Linf)
\begin{tabular}{lllrrrr}
\toprule
\textbf{Model} & \textbf{Dataset} & \textbf{Task} & \textbf{Acc.} & \textbf{Drop} & \textbf{MCC} & \textbf{ASR} \\
\midrule
Standard & Bot-IoT & Binary & 0.9341 & 6.59 & 0.1000 & 0.0658 \\
Standard & Bot-IoT & Multiclass & 0.3226 & 55.06 & 0.0119 & 0.0192 \\
Standard & CICIDS & Binary & 0.8418 & 9.52 & 0.2337 & 0.8517 \\
Standard & CICIDS & Multiclass & 0.7778 & 15.65 & 0.0984 & 0.8700 \\
Standard & UNSW-NB15 & Binary & 0.4603 & 33.46 & -0.1321 & 0.3146 \\
Standard & UNSW-NB15 & Multiclass & 0.1431 & 54.49 & 0.0160 & 0.1156 \\
\midrule
Bloom & Bot-IoT & Binary & 0.8125 & 18.75 & 0.1152 & 0.1874 \\
Bloom & Bot-IoT & Multiclass & 0.3955 & 40.93 & 0.0144 & 0.0100 \\
Bloom & CICIDS & Binary & 0.8412 & 5.69 & 0.2047 & 0.8666 \\
Bloom & CICIDS & Multiclass & 0.7725 & -17.76 & 0.0705 & 0.8760 \\
Bloom & UNSW-NB15 & Binary & 0.4846 & 27.28 & -0.0525 & 0.4325 \\
Bloom & UNSW-NB15 & Multiclass & 0.1569 & 32.73 & 0.0206 & 0.1095 \\
\bottomrule
\end{tabular}
 
% Table 7 (same filter)
\begin{tabular}{lllrr}
\toprule
\textbf{Dataset} & \textbf{Task} & \textbf{Class} & \textbf{Standard} & \textbf{Bloom} \\
\midrule
CICIDS & Multiclass & Bots & 0.91 & 0.90 \\
CICIDS & Multiclass & Web attacks & 0.91 & 0.91 \\
CICIDS & Multiclass & Port scanning & 0.90 & 0.91 \\
CICIDS & Multiclass & Brute force & 0.90 & 0.90 \\
CICIDS & Multiclass & DDoS & 0.89 & 0.89 \\
CICIDS & Binary & Malicious & 0.85 & 0.87 \\
CICIDS & Multiclass & DoS & 0.84 & 0.85 \\
\midrule
UNSW-NB15 & Binary & Malicious & 0.31 & 0.43 \\
UNSW-NB15 & Multiclass & DoS & 0.18 & 0.20 \\
UNSW-NB15 & Multiclass & Analysis & 0.18 & 0.25 \\
UNSW-NB15 & Multiclass & Backdoor & 0.17 & 0.23 \\
UNSW-NB15 & Multiclass & Worms & 0.17 & 0.14 \\
UNSW-NB15 & Multiclass & Exploits & 0.15 & 0.16 \\
UNSW-NB15 & Multiclass & Fuzzers & 0.15 & 0.18 \\
UNSW-NB15 & Multiclass & Reconnaissance & 0.11 & 0.10 \\
UNSW-NB15 & Multiclass & Shellcode & 0.09 & 0.08 \\
UNSW-NB15 & Multiclass & Generic & 0.07 & 0.03 \\
\midrule
Bot-IoT & Binary & Malicious & 0.07 & 0.19 \\
Bot-IoT & Multiclass & Reconnaissance & 0.04 & 0.03 \\
Bot-IoT & Multiclass & DDoS & 0.02 & 0.01 \\
Bot-IoT & Multiclass & DoS & 0.02 & 0.01 \\
Bot-IoT & Multiclass & Theft & 0.00 & 0.00 \\
\bottomrule
\end{tabular}
 
% Table 5 (same filter)
\begin{tabular}{llrrrr}
\toprule
\textbf{Model} & \textbf{Perturbation} & \shortstack{\textbf{Acc. drop}\\\textbf{(pp)}} & \textbf{MCC} & \textbf{ASR} & \textbf{FAR} \\
\midrule
Standard & FGSM & 35.89 & -0.0206 & 0.4786 & 0.5520 \\
Standard & Random $L_2$ & 27.02 & 0.0521 & 0.3246 & 0.6117 \\
Standard & Random $L_\infty$ & 24.48 & 0.1325 & 0.3152 & 0.5565 \\
\midrule
Bloom & FGSM & 24.58 & -0.0146 & 0.5167 & 0.5160 \\
Bloom & Random $L_2$ & 15.69 & 0.0585 & 0.3681 & 0.5462 \\
Bloom & Random $L_\infty$ & 13.54 & 0.1425 & 0.3563 & 0.5075 \\
\bottomrule
\end{tabular}
 
 

